Falcon-H1: A Family of Hybrid-Head Language Models Redefining Efficiency and Performance

In this report, we introduce Falcon-H1, a new series of large language models (LLMs) featuring hybrid architecture designs optimized for both high performance and efficiency across diverse use cases. Unlike earlier Falcon models built solely on Transformer or Mamba architectures, Falcon-H1 adopts a parallel hybrid approach that combines Transformer-based attention with State Space Models (SSMs), known for superior long-context memory and computational efficiency. We systematically revisited model design, data strategy, and training dynamics, challenging conventional practices in the field. Falcon-H1 is released in multiple configurations, including base and instruction-tuned variants at 0.5B, 1.5B, 1.5B-deep, 3B, 7B, and 34B parameters. Quantized instruction-tuned models are also available, totaling over 30 checkpoints on Hugging Face Hub. Falcon-H1 models demonstrate state-of-the-art performance and exceptional parameter and training efficiency. The flagship Falcon-H1-34B matches or outperforms models up to 70B scale, such as Qwen3-32B, Qwen2.5-72B, and Llama3.3-70B, while using fewer parameters and less data. Smaller models show similar trends: the Falcon-H1-1.5B-Deep rivals current leading 7B-10B models, and Falcon-H1-0.5B performs comparably to typical 7B models from 2024. These models excel across reasoning, mathematics, multilingual tasks, instruction following, and scientific knowledge. With support for up to 256K context tokens and 18 languages, Falcon-H1 is suitable for a wide range of applications. All models are released under a permissive open-source license, underscoring our commitment to accessible and impactful AI research.

==> sections/74b_training_data.tex <==
\section{Training Data} 

\subsection{English Web Data}

To enhance the performance of the large language model and optimize the training process, we introduced additional filtering steps to reduce noise and improve the quality of the initial English dataset. This dataset, comprising 15 TT of publicly available web data, includes a large amount of irrelevant or low-quality content. Filtering these data is an important step in ensuring that the training process is efficient and stable. 

One of the primary reasons for implementing this filtering step is to reduce the overall size of the dataset, which in turn decreases the pre-training time and computational cost. By minimizing the amount of redundant and noisy data, we can achieve a more resource-efficient training process, which is particularly important given the parameter count. In addition to reducing costs and time, filtering the dataset has a direct impact on improving the LLM performance. Large datasets containing substantial noise can introduce irrelevant or contradictory information, which negatively affects the model's ability to learn effectively and generalize well across tasks. By eliminating these low-quality samples, we observed a stable training with fewer spikes in the loss curve.

\textbf{Choosing the best model for the task.} We took a small sample of web data consisting of about 1000 documents and manually labeled them into two categories: low-quality and high-quality documents. Afterwards, we used multiple LLMs in the 7-10B size range to classify the same dataset, and compared the classification scores (using accuracy and F1 score). Finally, we chose the best LLM for the task that yielded 76\% accuracy when compared to the manually labeled dataset.

\textbf{Labeling the dataset.} After splitting each document into smaller paragraphs, we passed each paragraph through the LLM and gave it a quality score between [0-1]. The process of labeling 15 TT of web data took approximately 540,000 GPU Hours (using 1500 H100 and A100 GPUs for 15 days).

\textbf{Sampling a smaller high-quality dataset.} After labeling the entire dataset, we had a list of quality scores for each document. There were multiple sampling strategies to consider: using the minimum, maximum, or mean quality scores for each document as a metric. We then compare this metric with some threshold, and if it is higher, the document is kept. We finally chose the most aggressive strategy, using the minimum value of the quality scores for a given document as a metric, and discarded approximately 30\% of the data.

\subsection{Synthetic English Data}

In terms of synthetic English training data, we employ both external sources but also a substantial quantity of in-house generated data.

\textbf{Puzzle game data.} We generate synthetic data for puzzle game environments, structured as discrete 2D grids composed of interconnected rooms described by natural language, containing obstacles (e.g., walls, doors), and various objects (e.g., keys, balls, boxes) with a unique set of properties (color, interaction). These elements, depending on their number/size, allow to vary the complexity of the puzzle environment. Agents are given missions in natural language, and asked to execute a series of atomic actions. Each agent has access to six discrete operations: turning left, turning right, moving forward, picking up objects, dropping objects, and toggling (opening or closing) doors or boxes. More details are given in Section~\ref{app:puzzle data}. Following this setup, 70.5 GT of puzzle game data was synthetically generated.

\textbf{Nemotron-CC dataset}. Starting with the 8k context-length training stage of the model, we used three \textit{high-quality} synthetic data subsets from the Nemotron-CC dataset \citep{nemotron-cc}: ``Diverse Question-Answer (QA) pairs'', ``Extract knowledge'' (a rewrite the document focusing on knowledge retention and removing uninformative content), and ``wrap medium'' (the latter corresponding to a Wikipedia-style prompt rewrite of web samples resulting in high-quality data). For the QA pairs subset, the original seed documents were chunked before generating the QA pairs, however we concatenate the seed data chunks to recover the original document and place all the QA pairs at the end, which helps obtain samples with longer context length.

\textbf{High school math dataset.} To improve the basic math skills of the model, we generated raw question-solution pairs using the codebase from DeepMind's mathematics dataset \citep{dm_math}. Since the language in these questions is rudimentary and the solutions contain only the final answers without any steps, we first rephrased the questions to enhance vocabulary, then applied a similar method to STaR \citep{star} to generate the correct chain-of-thought solutions. Namely, we kept the generated solution if the predicted final answer matched the true answer; otherwise, we provided the true answer as a hint, then regenerated the solution and kept it if it was correct. We used the same model to generate the solutions and evaluate the correctness of the final answers. Subsequently, these data were translated into multiple languages.

\textbf{Synthetic textbooks.} To increase the breadth and depth of knowledge in both STEM and non-STEM domains, we generated synthetic textbooks to complement the human-written data. The seed data for each synthetic textbook is a topic hierarchy where the focus is on the most fine-grained one. We carefully selected more than 30K topic hierarchies extracted from Wikipedia, where we maximized knowledge coverage and reduced overlaps. More specifically, to build each topic hierarchy, we started from a list of 99 root categories (see Table~\ref{tab:wikipedia-categories-synthetic}, then crawled the Wikipedia category trees horizontally up to a vertical depth of 5 (or less if the end node was an article rather than a category); finally, we deduplicated and removed irrelevant topics from resulting branches. For each topic hierarchy, we first generated the table of contents, then for each unit, we included a thorough explanation of the topic, relevant examples, and diverse exercises. Similar ideas have been explored by Phi-1.5 \citep{phi1.5}, Cosmopedia \citep{cosmopedia}, etc. 

\textbf{Augmented topic-specific data.} Finally, for later training stages, to further increase model performance in STEM and non-STEM domains, we produce in-house synthetic training data using as seed data either subsets of the FineFineWeb dataset \citep{finefineweb} (38 topics, as detailed in Table~\ref{tab:ffw2-categories-synthetic}) or in-house web-crawl data (for specific topics such as Mathematics and Business).

\subsection{English data from curated sources}

For the initial training stages, we included the same collection of curated corpora consisting of conversations (general and technical), books, scientific publications and technical reports, encyclopedias, and patents, as used for previous Falcon models \citep{falcon, falcon11b}. This English data was harvested from sources such as Project Gutenberg \cite{gutenberg}, ArXiv, PubMed Central, PubMed Abstracts, Reddit \citealt{baumgartner2020pushshift}, stackexchange, HackerNews, Wikipedia \citep{wikidumps}, OpenSubtitles -- \citealt{tiedemann-2016-finding}, Ubuntu IRC, YouTube, StackOverflow), EuroParl \citep{europarl},  USPTO Patents. For later  training stages, we added English data from the FreeLaw, S2ORC-abstracts, S2ORC-central and Phil Papers datasets curated in TxT360 \citep{txt360}, and more specialized datasets such as \citet{gardian}.

\subsection{Multilingual web dataset}

Although mainly trained for the English language, the Falcon3.1-74B model also supports 16 other languages: Czech (cs), German (de), Spanish (es), French (fr), Hindi (hi), Italian (it), Japanese (ja), Korean (ko), Dutch (nl), Polish (pl), Portuguese (pt), Romanian (ro), Russian (ru), Swedish (sv), Urdu (ur), Chinese (zh). A fixed proportion between these languages was kept throughout the entire pre-training stages, as shown in Table~\ref{tab:ml_proportions_training}. The proposed distribution does not directly reflect the natural occurrence of data in these languages in CommonCrawl, being a compromise between data availability and language representation. The proportion was further adjusted for the decay stage, in an attempt to increase the contribution of under-represented languages.

\begin{figure}[t!]
    \centering
    \includegraphics[width=\textwidth]{figures/ml_distribution_74b.pdf}
    \caption{Relative proportions (expressed in \%) between the 16 languages making up the multilingual web-sourced component of the Falcon3.1-74B dataset, for (a) pre-training and (b) decay stages. Distribution of multilingual data by (c) source type. ISO 639 language codes are used as follows: Czech (cs), German (de), Spanish (es), French (fr), Hindi (hi), Italian (it), Japanese (ja), Korean (ko), Dutch (nl), Polish (pl), Portuguese (pt), Romanian (ro), Russian (ru), Swedish (sv), Urdu (ur), Chinese (zh).}
    \label{fig:ml_proportions_training}
\end{figure}

\begin{table}[ht]
 \caption{Relative proportions (expressed in \%) between the 16 languages making up the multilingual component of the Falcon3.1-74B pre-training web-sourced dataset. ISO 639 language codes are used as follows: Czech (cs), German (de), Spanish (es), French (fr), Hindi (hi), Italian (it), Japanese (ja), Korean (ko), Dutch (nl), Polish (pl), Portuguese (pt), Romanian (ro), Russian (ru), Swedish (sv), Urdu (ur), Chinese (zh).}
  \centering
  \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c}
    \toprule
    \textbf{Language} & \textbf{cs} & \textbf{de} & \textbf{es}  & \textbf{fr} & \textbf{hi} & \textbf{it} & \textbf{ja}  & \textbf{ko} & \textbf{nl} & \textbf{pl} & \textbf{pt}  & \textbf{ro} & \textbf{ru} & \textbf{sv} & \textbf{ur}  & \textbf{zh} \\
    \midrule
    \textbf{Pre-training} & 1.5 & 10 & 18 & 15.4 & 2 & 5 & 10 & 1 & 2.5 & 3 & 7.5 & 2 & 10 & 2 & 0.1 & 10 \\
    \midrule
    \textbf{Decay} & 3 & 10 & 10 & 10 & 3 & 9 & 9 & 3 & 3 & 3 & 10 & 3 & 9 & 3 & 3 & 9 \\
    \bottomrule
  \end{tabular}
  \label{tab:ml_proportions_training}
\end{table}

\textbf{Main data sources.} In terms of sources, 89.9\% of the multilingual data used in pre-training was web-sourced from CommonCrawl, with an additional 5.7\% being news excerpts from CCNews \cite{ccnews}, also originating from CommonCrawl; finally only 4.4\% of the data was from high-quality curated or academic sources, such as Wikipedia \citep{wikidumps}, academic pre-prints (ArXiv, PubMed Central, etc.), online conversation forums (Reddit -- \citealt{baumgartner2020pushshift}, HackerNews, OpenSubtitles -- \citealt{tiedemann-2016-finding}, Ubuntu IRC, YouTube, StackOverflow), open-source texts \cite{gutenberg}, public datasets containing data in the languages of interest \citep{europarl, gardian, makhzan} and closed-source datasets. The above distribution was followed throughout the pre-training. However, for decay the contribution of web data was reduced to roughly 50\%, and the high-quality data was further filtered, either by topic (see Table~\ref{tab:multilingual-hq-decay-categories}) or by source reputation (for news excerpts). For the final training stages we also employed a small amount of machine-translated (and human-validated) in-house generated synthetic math data, covering 12 languages, following an approach suggested in \cite{grattafiori2024llama3herdmodels}.

\textbf{CC extraction and coverage.} The multilingual web data was largely extracted directly from CommonCrawl. The language identification was initially done at HTML level using the \textit{pycld2} library, then re-identified using the multilingual \textit{fasttext} language classifier after HTML extraction with the \textit{trafilatura} library. The data was then divided in five parts of similar size, each consisting of 4-13 dumps dating between 2012 to mid-2024. Note that all available dumps from the interval 2022 to August 2024 were fully covered, with dumps from the 2012 to 2021 interval being randomly selected, as these tend to contain considerably less multilingual data.

\textbf{Data processing pipeline.} For processing the multilingual web data, following \citet{falcon11b}, we used the same heuristics-based data processing pipeline from \citet{refinedweb}, manually tuning the parameters and stop words used for Gopher Quality filtering \citet{gopher}, as well as the matching patterns for line-wise quality filtering, for each respective language. Afterwards, we split the data in multiple parts (two to five, depending on the language), and MinHash deduplication was applied to each part for each language, in an attempt to mimic the data strategy employed in constructing the FineWeb dataset \cite{fineweb-neurips}, where only near-deduplication was applied per dump. As multilingual data extracted from one dump is substantially less than that extracted for English, we did this at part level, with each part covering several dumps. More aggressive deduplication strategies (such as global MinHash deduplication, inter-dump URL-based deduplication, or string level exact deduplication) were not applied.

\textbf{Toxicity filtering.} All multilingual data was passed through a rule-based toxicity filtering process, using a human curated list of "(very) bad words". An initial list of words for each language was proposed to 1-3 native/proficient speakers, who assigned a grade from 0 to 2 to each word (0 meaning non-toxic, 1 potentially toxic depending on context, 2 always toxic). Finally, documents were filtered using a formula based on the number of such words detected in a document and a threshold for the cumulative toxicity grade, the formula being adjusted based on human feedback.

\textbf{Safety filtering.} Starting with our 8k context length pre-training stage, we also applied LLM-based safety filtering for data in supported languages: French, German, Hindi, Italian, Portuguese, and Spanish. For this purpose we used Llama-Guard-3-8B \cite{grattafiori2024llama3herdmodels}, with an English prompt only covering 9 of the 14 supported hazard categories (``Violent Crimes'', ``Non-Violent Crimes'', ``Sex Crimes'', ``Child Exploitation'', ``Defamation'', ``Indiscriminate Weapons'', ``Hate'', ``Self-Harm'', ``Sexual Content''). Each document was split into chunks containing less than 300 words, then each chunk was labeled as ``safe'', ``unsafe'' or ``undetermined'' (if the model failed to produce one of the previous two labels). Finally, only documents where all the chunks were labeled as ``safe'' passed the safety filtering. Across the six languages, we obtain the following percentages for samples that pass the safety filtering, measured as tokens in ``safe'' documents versus all tokens in the given range: $\sim95\%$ below 4k, $\sim80\%$ for 4-8k, $\sim76\%$ for 8-16k, and $\sim57\%$ above 16k. We hence observe two caveats in our chosen safety filtering strategy; first, a clear bias exists against longer documents which can be rejected only due to one unsafe paragraph (e.g., an unsavory comment following a good quality article); secondly, this strategy can prove too aggressive for lower-resource languages. In these cases, one could consider just eliminating the unsafe chunks as an alternative approach.

\textbf{Additional web data sources.} For a few languages, our internal data extraction efforts did not yield the desired number of tokens, particularly for longer context length ranges. For these cases, we supplemented with data from public multilingual datasets: part of the Hindi, Korean and Urdu data was sourced from CulturaY \citep{culturay}, and finally part of the Dutch, Romanian, Swedish, Korean and Urdu web data was also sourced from FineWeb2 \citep{fineweb2}; the same internal data processing pipeline for the respective languages was applied to these external data sources, to ensure quality alignment. The final multilingual dataset from web sources for the 16 languages used in pre-training amounted to over 1600 GT (billion tokens).

\subsection{Code data}
In order to increase the model's capabilities for a wide range of downstream applications, we curated an extensive code dataset for Falcon pre-training. It can be split into 3 main components that are used in different stages of training: the file-level corpus, the repo-level corpus, and the High Quality (HQ) code corpus.

\textbf{File-level corpus.} \label{file-level-code}
As most extensive code data source, we have an internally scraped and curated dataset, that comprehends a total of 620GT (specify GigaTokens if not already done) of code files, covering 67 programming languages, listed in \ref{appendix:programming_langs}. These samples are obtained from GitHub repositories created up to May 2024, as well as from Notebooks from the Meta Kaggle Code dataset.\footnote{\url{https://www.kaggle.com/datasets/kaggle/meta-kaggle-code}}

The notebooks have first been converted to scripts, using the JupyText library,\footnote{\url{ https://jupytext.readthedocs.io/}} then all file-level samples are processed through heuristic filtering \citep{stackv2}. Language labeling have been performed following \citep{refinedweb}, retaining samples classified as one of the 17 considered languages, with a lowered threshold of 0.15 for acceptance, as natural language in idioms other than English is usually limited to comments. Fuzzy deduplication has been performed with MinHash + Local Sensitive Hashing (LSH) \citep{MinHash}, computing 256 hashes per documents, with 5-grams and 0.85 Jaccard Similarity. Personally Identifiable Information (PII) entities, including e-mails and IP addresses, have been redacted with a pipeline inspired from DataTrove\footnote{\url{ https://github.com/huggingface/datatrove/blob/main/src/datatrove/pipeline/formatters/pii.py}} and replaced by >>EMAIL\_ADDRESS<<, >>IP\_ADDRESS<<. The same formatting for PIIs is applied to the whole pre-training corpus, with the exception of the English Web data, since the FineWeb dataset was already pre-processed in that regard.
This dataset represent the code source used in stages 1,2 and 3 of pre-training.

\textbf{Repo-level corpus.} In stage 4, given the extension of the context length, we introduce repo-level code samples \cite{deepseekcoder} \citep{qwencoder}. Training samples are obtained by concatenating all the single files in the repository, in order to allow cross-file code comprehension. 
For this dataset, MinHash deduplication is performed before filtering and at repository level, in order to not interfere with the repository cross-file logic. At deduplication step, files are concatenated in alphabetic order, to ensure effective identification of duplicates. Then, files are shuffled in order to reduce bias and ensure a robust representation. This results in a 170GT long-context code corpus.

\textbf{High quality code corpus}. For the annealing stage, we produce a HQ code corpus, starting from file-level and repo-level code datasets and running code quality classifiers over them. For programming languages other than Python, we employ a CodeBert-based code snippet classifier\footnote{\url{ https://huggingface.co/devngho/code_edu_classifier_v2_microsoft_codebert-base}} that supports 21 programming languages (see the full list in \ref{appendix:code_classifier}). Samples in these languages are included in the HQ corpus if their predicted quality score is at least 3. For Python samples, we apply an additional layer of validation by using both this multilingual classifier and the specialized python-edu-scorer.\footnote{\url{ https://huggingface.co/HuggingFaceTB/python-edu-scorer}} For each Python sample, we calculate the minimum score between the predictions of these two classifiers and include the sample in the HQ corpus only if this minimum score is at least 3. This ensures that Python samples meet the quality standards of both classifiers, which guarantees the educational quality of the selected snippets. This process produces 42GT of HQ file-level samples and 24GT of HQ repo-level samples.
Moreover, at this stage, we introduce the OpenCoder annealing corpus\cite{opencoder}, including its algorithmic corpus, synthetic question answering and synthetic code snippet datasets.\footnote{\url{ https://huggingface.co/datasets/OpenCoder-LLM/opc-annealing-corpus}} The pre-processing approach is the same as \ref{file-level-code}.


\subsection{Math Data}
 We use the following dedicated math datasets, along with the question-answer pairs generated from them, which we found further improved the model's performance on math-related tasks:
 \begin{itemize}
     %\item Proof-Pile-2 \citep{proofpile2}, consisting of mathematics data extracted from CommonCrawl, academic preprints and algebraic code sources, deduplicated using MinHash and lightly filtered to align with our other data sources. 
     \item Open-source datasets including Proof-Pile-2 \citep{proofpile2}, FineMath \citep{finemath}, InfiMM-WebMath-40B \citep{infimm-math} and OpenCoder FineWeb math corpus \citep{Huang2024OpenCoderTO}, which mainly consist of mathematics data extracted and filtered from Common Crawl.
     \item A dataset consisting of web math retrieved from both RefinedWeb \citep{refinedweb} and FineWeb \citep{fineweb} combined, using a fastText classifier \citep{fasttext} trained on web data from OpenWebMath \citep{openwebmath}, loosely following the methodology presented in the first stage of DeepSeekMath \citep{deepseekmath} data collection pipeline.
     \item A freshly crawled math dataset targeting top domains containing mathematics information; the seed domains were obtained by following the general strategy presented in the second stage of \citep{deepseekmath} data collection pipeline; the crawled data was then processed using a pipeline similar to that used for web and code data, loosely adapted for math data.
\end{itemize}

% Add with new datasets

\subsection{Multi-domain data}

To increase the model's multitask accuracy across both Humanities and STEM domains in later training stages, we curated English data covering both more general topics such as art, education, sports, science and technology, and specific topics such as biology, chemistry, computer science, geography, geology, history, mathematics, medicine, and physics. This data was decontaminated following the methodology described in \citet{cosmopedia}, with respect to the following benchmarks: IFEval \citep{ifeval}, BBH \citep{bbh}, MATH level 5 \citep{math}, GPQA \citep{gpqa}, MuSR \citep{musr}, MMLU-PRO \citep{mmlu-pro}, GSM8K \citep{gsm8k}. In order to preserve more training data from longer samples, when contamination was detected, a five-paragraphs long chunk containing the contaminated text was dropped from the larger sample, rather then directly rejecting the sample.

\subsection{Long Context Data}
To support long-context learning and evaluation, we construct specialized datasets that reflect realistic long-range dependencies in both natural language and code. This data is used during training of the model with extended context windows (up to 256k tokens), ensuring it is exposed to and tested on tasks that require reasoning over distant parts of the input.

\textbf{Fill In The Middle Data (FIM).} We create FIM-style datasets by leveraging naturally long documents, such as books and textbooks, ranging from 128k to 256k tokens. From these, we randomly remove one or more sections or subsections—typically at the chapter or heading level—to simulate realistic missing content scenarios. The removed content becomes the target for infill, while the remaining document is used as the prefix and suffix.

We apply this same methodology to code data, focusing on repo-level datasets. In code-specific examples, we may remove an entire function, module, or even an entire file implementation from the middle of the context, depending on the structure of the repository. This generates a rich and challenging FIM dataset that mirrors real-world use cases, such as understanding codebases with missing or incomplete components.

\begin{tcolorbox}[title=FIM format, colback=gray!5, colframe=tiipurple, fonttitle=\bfseries] \texttt{\textgreater{}\textgreater{}PREFIX\textless{}\textless{} {\{text pref\}} \textgreater{}\textgreater{}SUFFIX\textless{}\textless{} {\{text suff\}} \textgreater{}\textgreater{}MIDDLE\textless{}\textless{} {\{text mid\}}\textless{}\textbar{}endoftext\textbar{}\textgreater{}} \end{tcolorbox}

\textbf{Summarization, long context QA} @Puneesh 

==> sections/draft.tex <==
%========================================================
\section*{Appendix A Dynamical Origin of Loss Spikes in State–Space Models}
\label{app:dynamics}

Below we derive, from first principles, why the Mamba–style state–space module can
enter an unstable limit cycle when  
(a) the network is \emph{wide} (many heads, large hidden dimension) and  
(b) both short‐ and long‐range dependencies are simultaneously important to the language‐model objective.

%--------------------------------------------------------
\subsection*{A.1 SSM recurrence and notation}

For a single head, let the hidden state at discrete time \(t\) be
\(
\mathbf h_t \in \mathbb R^{N}
\)
and the input embedding be
\(
\mathbf x_t \in\mathbb R^{P}.
\)
The \emph{continuous-time} SSM is  
\(
\dot{\mathbf h}(t)\;=\;A\,\mathbf h(t)\;+\;B\,\mathbf x(t),\;
\mathbf y(t)\;=\;C\,\mathbf h(t),
\)
where \(A\) is diagonal and \(B,C\) are vectors.
After discretisation with a learned, {\smaller\(\text{log1pexp}\)} time‐step  
\(
\tilde{dt}_t=\log\!\bigl(1+e^{dt_t}\bigr)
\)
and log-transition parameter \(A_{\log}\),
the forward recurrence used by Mamba is
\begin{equation}
\label{eq:discrete-recurrence}
\mathbf h_{t}
\;=\;
e^{-e^{A_{\log}}\tilde{dt}_{t}}\;\mathbf h_{t-1}
\;+\;
\tilde{dt}_{t}\,B\,\mathbf x_{t},
\qquad
\mathbf y_t \;=\;C^{\!\top}\mathbf h_t.
\end{equation}
For compactness define
\[
\overline{A}_t \;=\; e^{-e^{A_{\log}}\tilde{dt}_t}
\quad\text{and}\quad
\beta_t \;=\; \tilde{dt}_t\,B.
\]
Unfolding \eqref{eq:discrete-recurrence} gives the mixing matrix
\begin{equation}
\label{eq:Mts}
\boxed{%
M_{ts} \;=\; C^{\!\top}\beta_s
        \prod\nolimits_{i=s+1}^{t}\overline{A}_i},
\qquad
\mathbf y_t \;=\;\sum_{s\le t} M_{ts}\,\mathbf x_s.
\end{equation}

%--------------------------------------------------------
\subsection*{A.2 Gradient structure}

The scalar loss \(\mathcal L=\sum_{t}\ell_t(\mathbf y_t)\) is a function of all \(M_{ts}\),
hence of every \(dt_i\) and \(A_{\log}\).
Differentiating \eqref{eq:Mts}:

\paragraph{Gradients w.r.t.\ the \textbf{write gate} \(dt_s\).}
For \(s<t\),
\[
\frac{\partial \log M_{ts}}{\partial dt_s}
\;=\;
\underbrace{%
\frac{\partial\log\tilde{dt}_s}{\partial dt_s}}_{+\;} % sign
\;-\;
\sum_{i=s+1}^{t}
\underbrace{%
e^{A_{\log}}\,
  \frac{\partial\tilde{dt}_i}{\partial dt_i}\;
  \Bigl[\mathbb I\{i=s\}\Bigr]}_{0\text{ if }i\!\neq\! s}.
\]
Thus only the first (write) term survives:
\[
\frac{\partial \mathcal L}{\partial dt_s}
\;=\;
\frac{\partial\tilde{dt}_s}{\partial dt_s}\!
\Bigl[\!
  \frac{\partial \mathcal L}{\partial\tilde{dt}_s}
  \;-\;
  e^{A_{\log}}
  \sum_{t>s}
    \frac{\partial \mathcal L}{\partial \overline{A}_t}
\Bigr].
\tag{A.1}
\]

\paragraph{Gradients w.r.t.\ the \textbf{decay log-rate} \(A_{\log}\).}
Using
\(
\partial\overline{A}_i/\partial A_{\log}
= -\,e^{A_{\log}}\tilde{dt}_i\,\overline{A}_i,
\)
\[
\frac{\partial \mathcal L}{\partial A_{\log}}
\;=\;
-\,e^{A_{\log}}
\sum_{i}
  \tilde{dt}_i\,\overline{A}_i\,
  \underbrace{\frac{\partial\mathcal L}{\partial\overline{A}_i}}_{\text{back‐prop signal}}.
\tag{A.2}
\]

\medskip
\noindent
\textbf{Antagonistic signs.}  
* Equation (A.1) receives a positive contribution from the write term at position \(s\) and (delayed) \emph{negative} contributions via \(\overline{A}_t\) at future positions.  
* Equation (A.2) aggregates \emph{only} negative contributions, pushing \(A_{\log}\) downward whenever the model tries to restore memory.

%--------------------------------------------------------
\subsection*{A.3 Why a small \(\delta dt\) becomes a large memory loss}

Consider perturbing a single time-step by \(\delta dt>0\).
The write factor grows \(\propto (1+\eta\delta dt)\) (linear), whereas each future
\(\overline{A}_i\) is multiplied by
\(\exp\{-e^{A_{\log}}\delta\tilde{dt}\}\) (exponential).
Over a span \(L\) tokens long,
\[
\prod_{i=1}^{L} \overline{A}'_i
\;=\;
\exp\!\Bigl[-e^{A_{\log}}\,
            \bigl(\tilde{dt}_1+\delta\tilde{dt}\bigr)
            -\dots-
            e^{A_{\log}}\,\tilde{dt}_L
       \Bigr]
\;=\;
e^{-e^{A_{\log}}\sum_i \tilde{dt}_i}\;
e^{-e^{A_{\log}}\delta\tilde{dt}},
\]
so the memory trace decays by an \emph{extra}
\(
e^{-e^{A_{\log}}\delta\tilde{dt}}
\).
For typical \(A_{\log}\approx 0\) and \(\delta\tilde{dt}=0.02\) this is a 2 % loss \emph{per step}, amounting to a factor two after \(L\!\simeq\!32\) steps.  
The optimiser therefore observes a modest write gain but a catastrophic context loss.

%--------------------------------------------------------
\subsection*{A.4 Feedback delay in a recurrent update}

Training with truncated BPTT of length \(T\) unfolds the network, accumulates the
gradients in (A.1)–(A.2), then applies a single joint update
\(
\theta\gets\theta-\eta\,m_1/\!\sqrt{m_2+\epsilon}
\)
for \(\theta=\{dt,A_{\log}\}\).
Because the damaging positive write gradient arrives \emph{one iteration} earlier than the restoring negative memory gradient, the update acts on stale information.  
In stiff directions (here, the write–forget axis) a one-step lag can shift the eigenvalues of the linearised system outside the unit circle, yielding an under-damped oscillator:

\[
\theta_{k+1}
\;=\;
\underbrace{%
\bigl[I-\eta H\bigr]}_{\substack{\text{eigenvalues}>\!1\\
\text{if }\eta\text{ too large}}}
\;\theta_k
\;+\;
O\!\bigl(\eta^2\bigr),
\]
where \(H\) is the Hessian.  
For Adam, moment adaptation further amplifies any burst in the squared gradient, so the effective step size \(\eta/\sqrt{m_2}\) \emph{increases} precisely when the system needs damping.

%--------------------------------------------------------
\subsection*{A.5 Width vs depth}

Let each head carry its own \((dt,A_{\log})\).  
For a fixed parameter budget \(D\!\cdot\!N\) (\(D=\) depth, \(N=\) hidden size), making the model \textbf{wide} multiplies the number of heads \(H\) and thus the dimensionality of the unstable write–forget subspace.  
The largest eigenvalue of the combined Jacobian grows roughly
\(
\lambda_{\text{max}}\;\sim\;1+\eta\,H\sigma^2,
\)
with \(\sigma^2=\text{Var}(\partial\mathcal L/\partial dt)\).
Beyond a critical \(H\) the trajectory diverges, whereas adding layers (greater \(D\)) deepens the chain of products \(\prod\overline{A}_i\), further dampening long-range gradients and acting as a stabiliser.

%--------------------------------------------------------
\subsection*{A.6 Mitigation via early \(\boldsymbol{dt}\) attenuation}

Clipping \(dt\) to \(dt_{\max}\) or multiplying it by a factor \(\alpha<1\) for the first \(K\) updates:

\[
dt^{\text{eff}}_t
\;=\;
\begin{cases}
\alpha\,dt_t & k\!\le\!K,\\
dt_t & k>K,
\end{cases}
\quad
0<\alpha<1,
\]
shrinks the Lipschitz constant of the write–forget map,
\(
L\;\propto\;
(1\!-\!\alpha)+\alpha\,e^{A_{\log}},
\)
below the critical value at which the eigenvalues cross the unit circle.
After the optimiser statistics have settled, the attenuation is removed; the system now operates in a smoother region of parameter space where opposing gradients can co-exist without explosive amplification.

\bigskip
\noindent
\textbf{Summary.}  
The training instability is a manifestation of a \emph{stiff, antagonistic} direction in the SSM parameter manifold: \(dt\) wants to be large for immediate write strength, while \(A_{\log}\) wants to be positive (small decay) to retain history.  
Their multiplicative coupling, delayed gradients, and moment-based optimisation create an under-damped feedback loop.  
Temporary damping of the write gate (\(\tilde{dt}\)) during the early phase reduces the Lipschitz modulus and restores stability without permanently limiting model capacity.

